An explicit predictor/multicorrector time marching with automatic adaptivity for finite-strain elastodynamics

We propose a time-adaptive predictor/multi-corrector method to solve hyperbolic partial differential equations, based on the generalized-$\alpha$ scheme that provides user-control on the numerical dissipation and second-order accuracy in time. Our time adaptivity uses an error estimation that exploits the recursive structure of the variable updates. The predictor/multicorrector method explicitly updates the equation system but computes the residual of the system implicitly. We analyze the method's stability and describe how to determine the parameters that ensure high-frequency dissipation and accurate low-frequency approximation. Subsequently, we solve a linear wave equation, followed by non-linear finite strain deformation problems with different boundary conditions. Thus, our method is a straightforward, stable and computationally efficient approach to simulate real-world engineering problems. Finally, to show the performance of our method, we provide several numerical examples in two and three dimensions. These challenging tests demonstrate that our predictor/multicorrector scheme dynamically adapts to sudden energy releases in the system, capturing impacts and boundary shocks. The method efficiently and stably solves dynamic equations with consistent and under-integrated mass matrices conserving the linear and angular momenta as well as the system's energy for long-integration times.

==> Arxiv 2/AlgebraicAspectsVMC2.tex <==
\section{Solution strategies and time-step size adaptivity}
\label{section:Implement}


\begin{figure} 
  \begin{center}
    \subfigure[(Interior) Gauss quadrature] {\includegraphics[width=.45\textwidth]{NonlumpedMass.pdf}}
    \hfill
    \subfigure[(Nodal) Gauss-Lobatto quadrature] {\includegraphics[width=.45\textwidth]{lumpedMass.pdf}}
  \end{center}
  \caption{Mass matrix sparsity structure for a tetrahedral mesh using different integration rules}
\label{Quadrature}
\end{figure}

This section discusses time adaptivity and efficient variable updates for our method. We perform all the numerical experiments using the open-source FEniCS environment~\cite{ alnaes2015fenics} using the FIAT package~\cite{ Kirby2004} to integrate with different quadratures.  We estimate the truncation error to update the time-step size dynamically as the simulation progresses as in~\cite{ GOMEZ20084333}
%
\begin{equation}
  F\left(e;\Delta t; \text{tol} \right) = \rho_{\text{tol}} \left( \frac{\text{tol}}{e} \right)^{\frac{1}{d}} \Delta t,
  \label{TimeUpdate}
\end{equation}
% 
where $ \rho_{\text{tol}}$ is a safety coefficient with the tolerance $\text{tol}$ taken from~\cite{ LANG1995223}, $d$ is the problem's spatial dimension and we estimate the truncation error $e$ using a summation expressed in terms of the update 
\begin{equation}
e = \frac{\| \delta \boldsymbol{u}^{k} \|_{L^2}}{\| \delta \boldsymbol{u}^{k-1}\|_{L^2}}  \ ,
\end{equation}
where $k$ is the term number of the updating formula.  In highly nonlinear problems, the time-step size can vary orders of magnitude to maintain the maximum eigenvalue of the amplification matrix lower than one. In our experience, the adaptive scheme avoids thousands of calculation steps while providing convergence at a low computational cost,  and no time-step bounding are needed since this is provided by the method itself. Algorithm~\ref{Alg1Adap} sketches the time marching scheme.  We make our explicit time-integrator attractive for engineering applications by using reduced integration for the mass matrix. Figure~\ref{Quadrature} shows the structure of a mass matrix calculated using different integration methods. Figure~\ref{Quadrature}(a) represents the sparsity obtained using Gauss quadrature, whereas Figure~\ref{Quadrature}(b) shows that, when we collocate integration points at the nodes; that is, we use a Gauss-Lobatto quadrature. Thus, the resultant mass matrix is diagonal. As a consequence, all updates only involve scalar-vector algebraic operations with a negligible computational cost. When we use the mass matrix integrated with Gauss-Lobatto quadrature as a preconditioner for the LGMRES solver, it converges in two iterations in serial computing. 	
% 
\begin{algorithm}[h]  
\SetAlgoLined
\KwData{$\boldsymbol{u}_n$, $\dot{\boldsymbol{u}}_n$, $\ddot{\boldsymbol{u}}_n$ and $\Delta t_{n+1}$}
\KwResult{$\boldsymbol{u}_{n+1}$, $\dot{\boldsymbol{u}}_{n+1}$, $\ddot{\boldsymbol{u}}_{n+1}$ and $\Delta t_{n+1}$}
 Initialize $ \boldsymbol{u}_n  = \boldsymbol{u}_0$, $ \dot{\boldsymbol{u}}_n = \dot{\boldsymbol{u}}_0$ and $\ddot{\boldsymbol{u}}_n = \ddot{\boldsymbol{u}}_0$ for $t_n = 0$\;
 \While{$t_{n} \leq t_{f}$}{
  Update Matrix $\mathbb{K}^{*} =  -  \frac{\alpha_{f} \gamma_{2} \Delta t^{2}}{\alpha_{m} } \mathbb{K}$ and Mass Matrix $\mathbb{M}$\;
  Update Vector $\bold{H} $ \;
  Compute $\delta \boldsymbol{u}^{1}_{n+1} = \text{solve} \left(\mathbb{M},  \mathbb{K}^{*} \cdot \bold{H}\right)$ \;
  Compute $\delta \boldsymbol{u}^{2}_{n+1} = \text{solve} \left(\mathbb{M},  \mathbb{K}^{*} \cdot \delta \boldsymbol{u}^{1}_{n+1}\right)$ \;
  $\vdots$ \\
  Compute $\delta \boldsymbol{u}^{k}_{n+1} = \text{solve} \left(\mathbb{M},  \mathbb{K}^{*} \cdot \delta \boldsymbol{u}^{k-1}_{n+1} \right)$ \;
  Compute error $e_{n+1} = \frac{\| \delta \boldsymbol{u}^{k}_{n+1} \|_{L^2}}{\| \delta \boldsymbol{u}^{k-1}_{n+1} \|_{L^2}}$ \;
  \eIf{$e_{n+1} \leq \text{tol}$}{
   Update Current time-step $t_{n} \leftarrow t_{n} + \Delta t_{n+1}$\;
   Update $\lJump \boldsymbol{u} \rJump_{n+1} = \sum^{k}_{j=1} \delta \boldsymbol{u}^{j}_{n+1}$ \;
   Update $\boldsymbol{u}_{n+1}$, $\dot{\boldsymbol{u}}_{n+1}$ and $\ddot{\boldsymbol{u}}_{n+1}$\;
   Update $\boldsymbol{u}_{n} \leftarrow \boldsymbol{u}_{n+1}$, $\dot{\boldsymbol{u}}_{n} \leftarrow \dot{\boldsymbol{u}}_{n+1}$ and $ \ddot{\boldsymbol{u}}_{n} \leftarrow \ddot{\boldsymbol{u}}_{n+1}$\;
   \If{$e_{n+1} < \text{tol}_{min}$}{
   Increase time-step $\Delta t_{n+1} \leftarrow F\left(e_{n+1};\Delta t_{n+1}; \text{tol}_{min}\right)$}
   }{
   Reduce time-step $\Delta t_{n+1} \leftarrow F\left(e_{n+1};\Delta t_{n+1}; \text{tol}\right)$\;
  }
 }
 \caption{Explicit update with time-step size adaptativity}
 \label{Alg1Adap}
\end{algorithm}




==> Arxiv 2/ConclusionsVMC2.tex <==
\section{Conclusions}
\label{section:Conclusions}

We introduce a new class of predictor/multicorrector time-marching techniques for explicit generalized-$\alpha$ methods. Our proposal has a cheap and robust error estimator that can guide adaptability even in the presence of sudden shocks to the system. Another key advantage of our predictor/multicorrector method is that our variable updates are explicit from $n$ to $n+1$ while evaluating the residual at $n+1$; we only factor the mass matrix to compute the explicit update, while we can control the residual at time $n+1$ as in implicit methods. We estimate the method's error by comparing the truncation terms of the update formula. This time-error estimator provides a robust quantity to guide the time-step size adaptivity, circumventing the lack of convergence of the nonlinear residual that characterizes explicit methods. 

Our explicit generalized-$\alpha$ method controls the high-frequency numerical dissipation. We analyze the method's stability regimes and determine the corresponding parameters to guarantee second-order accuracy in time and to maximize stability.  We demonstrate the method's performance (accuracy and efficiency) on various numerical examples. The first two confirm that our method delivers the optimal second-order convergence for linear and nonlinear hyperbolic equations. Next, we study large-deformation problems subject to sudden shocks that induce instantaneous energy releases. We study a twisted bar subject to gravitational loading that we release suddenly and the impact of a cylindrical tube onto a rigid wall. These examples show our time adaptability's ability to describe the dynamics of rubber-like hyperelastic material subject to sudden releases of potential or kinetic energies. The final example is a classical benchmark used in the community to analyze the momentum and energy conservation. The \textit{tossed ruler} problem shows that our method is energy stable when using consistent and lumping mass matrices to compute the variable update. We show that the predictor/multicorrector approach described is a suitable tool to correct the energy unbalance produced when Gauss-Lobatto quadrature, which is commonly used to obtain diagonal mass matrices in dynamic problems. 

In conclusion, our method is a computationally efficient and robust predictor/multicorrector method for real-life applications, where convergence is always guaranteed regardless of the problems' dynamics while accounting for shocks within the solution as well as from external loadings,  providing energy and momentum stable solutions. This is a key advantage when it is compared with other explicit time-marching methods, where the error is not a built-in quantity while it has to be computed using methods with different convergence order,  at the same time they dissipate energy and momentum when lumped mass matrices are used.



==> Arxiv 2/InsightVMC2.tex <==
\section{Predictor/multicorrector time integration}
\label{section:insight}

In this section, we introduce a predictor/multicorrector scheme based on the generalized-$\alpha$ philosophy. For this, we discuss the strong and weak forms of the time-dependent problem. Then, we introduce a time discretization to update the displacement and acceleration.

\subsection{Strong and weak formulations of a time-dependent problem}

Let $\mathcal{B}\subset \mathbb{R}^{d}$, where $d \in \left\lbrace 1,2,3\right\rbrace$ is the spatial dimension and $I \in \left[0,T \right]$ is the time interval. We consider the following wave equation:
%
\begin{equation}
  \left\{
    \begin{aligned}
      \ddot{{u}} - \Delta {u} &= {f}\left({x},t\right), &&
                                                               \text{in} \ \ \mathcal{B}\times I, \\ 
      {u}\left({x},t\right)  & = {u}_D,  && \text{on} \ \  \partial\mathcal{B} \times I,  \\
      {u} \left({x}, 0 \right) & = {u}_0,\quad\quad 
      \dot{{u}}\left({x}, 0 \right)  = \dot{{u}}_0,  && \text{on} \ \  \mathcal{B},
    \end{aligned}\right.
  \label{eq:HyperbolicPDE}
\end{equation}
%
where $x \in \mathcal{B}$ is the body's coordinate system, ${u} : \mathcal{B} \times I \rightarrow \mathbb{R}^{m}$, with $m \geq 1$, is the unknown field, $\ddot{{u}} \coloneqq \frac{\partial^{2} {u}}{\partial t^{2}} $ is its second time derivative and $\Delta u=\frac{\partial^2 u}{\partial x_i^2}$ its spatial Laplacian, ${f} : \mathcal{B} \times I \rightarrow \mathbb{R}^{m}$ is the source term, and $\partial\mathcal{B}$ denotes the spatial boundary of $\mathcal{B}$. The partial differential equation (PDE)~\eqref{eq:HyperbolicPDE}$_1$ is subject to ${u}_D$, ${u}_0$, and $\dot{{u}}_0$, the Dirichlet boundary~\eqref{eq:HyperbolicPDE}$_2$ and initial conditions ~\eqref{eq:HyperbolicPDE}$_3$, respectively.

Multiplying~\eqref{eq:HyperbolicPDE}$_1$ by a smooth weighting function ${v}$ in $\mathcal{V}$ that vanishes on $\partial \mathcal{B}$, and integrating by parts in space, we obtain:
%
\begin{align}
    \displaystyle \int_{I} \int_{\mathcal{B}} {v}  {f}  \
  d\mathcal{B}\ dt
  &=\displaystyle \int_{I} \int_{\mathcal{B}} \left( {v} \ddot{{u}}  -
    {v} \Delta {u}  \right) d\mathcal{B}\ dt,  
    = \int_{I} \int_{\mathcal{B}} \left( {v}  \ddot{{u}} + \nabla {v}
    \cdot \nabla {u} \right) d\mathcal{B}\ dt. \label{eq:HyperbolicPDEWeak2}
\end{align}
%
Using standard notation, we state that the above formulation is sufficient to ensure that all terms in~\eqref{eq:HyperbolicPDEWeak2} belong to  ${H}^1$ in space and ${L}^2$ in time. In this sense, the test space is
%
\begin{equation}
  \mathcal{V} \coloneqq {H}^{1}_{0}\left( \mathcal{B}\right) \coloneqq
  \left\lbrace  {v} \in {L}^2\left( \mathcal{B}\right)  |   \nabla {v}
    \in {L}^2\left( \mathcal{B}\right), {v} = 0 \in
    \partial\mathcal{B} \right\rbrace  
  \label{eq:HyperbolicPDEWeak3}
\end{equation}
%
Given~\eqref{eq:HyperbolicPDEWeak2}, then $\ddot{{u}}$ and ${f}$ belong to the dual space of the test space $\mathcal{V}^{\ast} = {H}^{-1}\left( \mathcal{B}\right)$. Thus, the trial space is
%
\begin{equation}
  \mathcal{U} \coloneqq \left\lbrace {u} \in \mathcal{V} \ \ | \ \
    \ddot{{u}} \in \mathcal{V}^{\ast},  {u} \left({x}, 0 \right) = {u}_0,
    \dot{{u}}\left({x}, 0 \right)  = \dot{{u}}_0,
      {u} = {u}_D \in  \partial\mathcal{B} 
  \right\rbrace . 
  \label{eq:HyperbolicPDEWeak4}
\end{equation}
%
where $  {u}_0, \dot{{u}}_0 \in {L}^2\left( \mathcal{B}\right).$

Finally, the weak problem reads: \textit{Given $ {f} \in \mathcal{V}^{\ast}$ a source term, find ${u} \in \mathcal{U}$ such that}
%
\begin{align}
  \displaystyle \int_{I} \left\langle  {v} , \ddot{{u}}  \right\rangle
  dt
  &= \displaystyle \int_{I} \left\langle {v} , {f}   \right\rangle dt
    - \int_{I} a\left(  {v} , {u} \right) dt,
  &     \forall v \in  \mathcal{V}
    \label{eq:HyperbolicPDEproblem}
\end{align}
% 
where $\left\langle \cdot , \cdot \right\rangle $ is the duality pairing between $\mathcal{V}$ and $\mathcal{V}^{\ast}$, $a\left( {v} , {u} \right) = \left( \nabla {v} , \nabla {u} \right)$ is a linear form with $\left( \cdot, \cdot \right)$ the inner product in ${L}^{2}\left( \mathcal{B}\right)$.

\subsection{Predictor/multicorrector time-marching method}

Herein, we describe our time-marching method. For this aim, we discretize the time domain $t_0<t_1<...<t_n<...<t_f$, defining a time-step $\Delta t_n=t_n-t_{n-1}$. Approximating ${u}\left(t_n\right)$ and $\ddot{{u}} \left( t_n \right)$, respectively, using ${u}_n$ and $\ddot{{u}}_n$, we can state (for more details, see,~\cite{chung1993time}): 
%
\begin{equation}
  \begin{aligned}
    t_{n+\alpha_f} &= t_{n} + \alpha_f \Delta t, \\
    {u}_{n+\alpha_f} &=  \displaystyle {u}_{n} + \alpha_{f}  \lJump {u} \rJump ,  \\
    \ddot{{u}}_{n+\alpha_m} &=  \displaystyle \ddot{{u}}_{n}
    + \alpha_{m}  \lJump \ddot{{u}} \rJump, 
  \end{aligned}
  \label{eq:EqGenAlpha1}
\end{equation}
%
where $\lJump  \bullet \rJump = \left(\bullet \right)_{n+1} - \left( \bullet \right)_{n}$ is the time increment of a certain field $\bullet$. Using a Taylor series in time, we have:
%
\begin{align}
  {u}_{n+1}  &=  \displaystyle \sum_{j = 0}^{\phi+1} \frac{{\Delta
               t}^{j}}{j !} \left.{\frac{\partial^j {u}}{\partial
               t^j}}\right|_{n} ,  
               \label{eq:EqGenAlpha2}
\end{align}
%
where $\phi$ is the expansion order. Substituiting~\eqref{eq:EqGenAlpha1} into~\eqref{eq:HyperbolicPDEproblem}, the semi-discrete problem reads: 
%
\begin{equation}
\left\langle {v}  ,  \ddot{{u}}_{n+\alpha_m} \right\rangle   =  \displaystyle \left\langle {v}  , {f}_{n+\alpha_f} \right\rangle  -  a \left( {v}  ,  {u}_{n+\alpha_f}  \right)    , \ \ \ \  \forall {v} \in  \mathcal{V}  \ .
\label{eq:HyperbolicPDEproblemGalpha}
\end{equation}
%
\begin{remark}
  We denote the last-term constant in~\eqref{eq:EqGenAlpha2} as $\gamma_{\phi}$, while its increment is
  \begin{align}
    \lJump {u} \rJump &= \displaystyle \sum_{j = 1}^{\phi}
                        \frac{{\Delta t}^{j}}{j !}
                        \left.{\frac{\partial^j {u}}{\partial
                        t^j}}\right|_{n} +  \ \gamma_{\phi} {\Delta
                        t}^{\phi} \left[\!\!\left[
                        {\frac{\partial^{\phi} {u}}{\partial
                        t^{\phi}}} \right]\!\!\right]  
                        \label{eq:EqGenAlpha3}
  \end{align}
  %
  For hyperbolic PDEs, we let $\phi = 2$,  
  \begin{align}
    \lJump {u} \rJump  &=  \Delta t \left( \dot{{u}}_{n} + \Delta t
                         \left( \frac{\ddot{{u}}_{n} }{2}  +
                         \gamma_{2} \lJump \ddot{{u}}  \rJump \right)
                         \right),
                         \label{eq:taylorhyper}
  \end{align}
  %
  while we compute the velocity as
  %
  \begin{align}
    \lJump \dot{{u}} \rJump  &=  \Delta t \left( \ddot{{u}}_{n} +
                               \gamma_{1} \lJump \ddot{{u}}  \rJump
                               \right). 
                               \label{eq:taylorhyper11}
  \end{align}
%
  In the literature, the coefficients $\gamma_1$ and $\gamma_2$ are usually denoted in the bibliography as $\gamma$ and $\beta$, respectively~\cite{ chung1993time}. We use this notation in the remainder of the paper. 
\end{remark}

\subsection{Update in terms of ${u}$}

We substitute~\eqref{eq:EqGenAlpha1} into~\eqref{eq:HyperbolicPDEproblemGalpha} and solving in terms of $u$, we have:
%
\begin{equation}
\displaystyle \left\langle {v}  , \ddot{{u}}_{n} + \alpha_{m}  \lJump \ddot{{u}} \rJump \right\rangle   =  \left\langle {v}  , {f}_{n+\alpha_f}  \right\rangle  -  a \left(   {v} ,  {u}_{n} + \alpha_{f}  \lJump {u} \rJump \right).  
\label{eq:Galphau1}
\end{equation}
%
We deduce a set of useful equations for different problems, let $a \left( {v} , {u}_{n} + \alpha_{f} \lJump {u} \rJump \right)$ be a nonlinear functional. In this sense, we can approximate it using a second-order Taylor series expansion as
%
\begin{equation}
a \left( {v} , {u}_{n} + \alpha_{f}  \lJump {u} \rJump  \right) \approx a \left(   {v} , {u}_{n} \right) + \alpha_{f} \ a' \left(   {v}  , \lJump {u} \rJump ;  {u}_{n} \right),
\end{equation}
%
where $a' \left(  {v} , \lJump \bullet \rJump  ;  \bullet_{n} \right) $ is the Gateaux derivative of $a \left(   {v}  , \bullet  \right)$, defined as
%
\begin{equation}
a' \left(  {v} , \lJump {u} \rJump  ;  {u}_{n} \right) = \frac{d}{d\epsilon} a \left( {v} , {u}_{n} + \epsilon  \lJump {u} \rJump  \right) \vert_{\epsilon=0},
\end{equation}
%
Then, combining this equation with~\eqref{eq:Galphau1} leads to:
%
\begin{equation}
  \displaystyle  \alpha_{m}  \left\langle {v} ,  \lJump  \ddot{{u}}
    \rJump  \right\rangle = \displaystyle - \alpha_{f} \  a' \left(
    {v}  ,  \lJump {u} \rJump ; {u}_{n}  \right) + \left\langle  {v}  ,
    {f}_{n+\alpha_f}  \right\rangle  - \left\langle  {v} ,
    \ddot{{u}}_{n} \right\rangle -  a \left(  {v} , {u}_{n}   \right), 
\end{equation}
%
which we can express in terms of $\lJump {u} \rJump$ using~\eqref{eq:EqGenAlpha2} as
%
\begin{equation}
  \displaystyle \left\langle  {v}  , \lJump  {u} \rJump \right\rangle
  =  \displaystyle - \frac{\alpha_f \Delta t^2 \beta}{\alpha_m} a'
  \left(   {v} ,   \lJump {u} \rJump;  {u}_{n}  \right) + \ell \left(
    {v} \right),   
  \label{eq:Galphau1bis}
\end{equation}
%
with
%
\begin{equation}
  \ell \left( {v} \right) = \displaystyle \frac{\beta \Delta
    t^{2}}{\alpha_m}    \displaystyle \left[ \left\langle {v} ,
      {f}_{n+\alpha_f}  \right\rangle - \left\langle  {v} ,
      \ddot{{u}}_{n}  \right\rangle -  a \left( {v} ,  {u}_{n}  ,
    \right) \right]  +  \left\langle {v} , \sum_{j = 1}^{2}
    \frac{{\Delta t}^{j}}{j !} \left.{\frac{\partial^j {u}}{\partial
          t^j}}\right|_{n}  \right\rangle. 
\label{eq:Galphau1bisbis}
\end{equation}
%
We write the time increment as $\lJump {u} \rJump^{k+1} = \lJump {u} \rJump^{k} + \delta {u}^{k+1}$ in~\eqref{eq:Galphau1bis}, and considering the left term an iteration ahead respect to the right-hand side, we obtain
% 
\begin{align}
    \displaystyle \left\langle {v}  ,  \lJump  {u} \rJump^{k+1}
    \right\rangle    &=  \displaystyle - \frac{\alpha_f \Delta t^{2}
                       \beta}{\alpha_m} a' \left(
                       {v} ,  \lJump {u} \rJump^{k} ; {u}_{n}  \right)
                       + \ell \left( {v} \right), 
\end{align}
%
which we can rewrite as
%
\begin{align}
    \displaystyle \left\langle  {v} , \delta {u}^{k+1}  \right\rangle
                     &= \displaystyle - \frac{\alpha_f \Delta t^{2}
                       \beta}{\alpha_m} {a}' \left(  {v}
                       , \lJump {u} \rJump^{k} ; {u}_n   \right) -
                       \left\langle {v}  ,  \lJump  {u} \rJump^{k}
                       \right\rangle  + \ell \left( {v} \right). 
\label{eq:Galphau2}
\end{align}
%
Now, we consider a spatial discretization for $\mathcal{V}$ and $\mathcal{U}$:
%
\begin{equation}
  {u}^{h} = \sum_{i=1}^{n} \Phi_i \mathbf{U}_{i}  \subset  \mathcal{U}
  , \ \ \text{and} \ \ {v}^{h} \in \spn \left\lbrace  \Psi_j
  \right\rbrace^{m}_{j=1} \subset  \mathcal{V}, 
\end{equation}
%
with $\Phi_i$ and $\Psi_j$ being appropriate trial and test functions, respectively, while $\mathbf{U}_{i}$ is the unknown vector. Therefore, we obtain the fully-discrete problem as:
%
\begin{equation}
  \begin{aligned}
    \displaystyle \mathbb{M} \cdot \delta  \mathbf{U}^{k+1}
    &= \displaystyle -  \frac{\alpha_{f} \Delta t^{2} \beta
    }{\alpha_{m} }  \mathbb{K} \cdot  \lJump   \mathbf{U} \rJump^{k} -
    \mathbb{M} \cdot \lJump  \mathbf{U} \rJump^{k}    +  \mathbf{L},
    \\ 
    \displaystyle \delta  \mathbf{U}^{k+1}
    &= \displaystyle \left( -  \frac{\alpha_{f}  \Delta t^{2}
        \beta}{\alpha_{m} } \mathbb{M}^{-1} \mathbb{K} - \mathbb{I}
    \right) \cdot \lJump  \mathbf{U} \rJump^{k}    +  \mathbb{M}^{-1}
    \cdot \mathbf{L}, \\ 
    \displaystyle \delta  \mathbf{U}^{k+1}
    &= \displaystyle \left( \mathbb{U} - \mathbb{I} \right) \cdot
    \lJump  \mathbf{U} \rJump^{k}    +  \mathbf{H}, 
  \end{aligned} 
  \label{eq:Galphau4}
\end{equation}
%
where $\mathbb{M}$ and $\mathbb{K}$ are the mass stiffness matrices defined as
%
\begin{align*}
  \mathbb{M}_{ij} &= \left\langle \Psi_i  , \Phi_j \right\rangle =
                    \int_{\mathcal{B}} \Psi_i \Phi_j  \ d \mathcal{B},
  &
    \mathbb{K}_{ij} &= a' \left( \Psi_i , \Phi_j ; {u}_n \right) \\
  \mathbf{H} &=  \mathbb{M}^{-1} \cdot \mathbf{L},
  & \mathbf{L} &= \ell \left( \Psi_j \right) \ ,
\end{align*}
%
$\mathbb{M}^{-1}$ is the inverse matrix of the mass matrix $\mathbb{M}$ and $\mathbb{U} = - \frac{\alpha_{f} \Delta t^{2} \beta}{\alpha_{m} } \mathbb{M}^{-1} \mathbb{K}$ is the updating matrix, with the identity matrix $\mathbb{I}$.  Starting from~\eqref{eq:Galphau4} and assuming that, for $k=0$ the variable increment is $\lJump \mathbf{U} \rJump^{0} = 0$, the first increment is
%
\begin{align}
    \delta \mathbf{U}^{1} =  \mathbf{H}  \qquad \Rightarrow \qquad
  \lJump \mathbf{U} \rJump^{1} = \mathbf{H} . 
  \label{eq:Galphau5}
\end{align}
%
Substituting $\lJump \mathbf{U} \rJump^{k}$ into~\eqref{eq:Galphau4}, one can readily compute the increment $\delta \mathbf{U}^{k+1} $ in a recursive manner as:
%
\begin{equation}
  \begin{aligned}
    \delta \mathbf{U}^{2} & = \mathbb{U} \cdot \mathbf{H}
    && \Rightarrow && \lJump \mathbf{U} \rJump^{2}
     = \left(\mathbb{I} + \mathbb{U}\right) \cdot \mathbf{H},\\
    \delta \mathbf{U}^{3} &= \mathbb{U}^{2} \cdot \mathbf{H}
    && \Rightarrow && \lJump \mathbf{U} \rJump^{3}
    = \left(\mathbb{I} + \mathbb{U} + \mathbb{U}^{2} \right) \cdot \mathbf{H}, \\
    &&& \ \, \vdots &&\\
    \delta \mathbf{U}^{N} &= \mathbb{U}^{N-1} \cdot \mathbf{H}
    && \Rightarrow && \lJump \mathbf{U} \rJump^{N}
    = \left(\mathbb{I} + \mathbb{U} + \mathbb{U}^{2} + ...
      + \mathbb{U}^{N-1} \right) \cdot \mathbf{H},
  \end{aligned} 
  \label{eq:recursiveu}
\end{equation}
%
Finally, the predictor/multicorrector updates the variable using an explicit generalized-$\alpha$ scheme as follows
%
\begin{equation}
  \boxed{
    \ \lJump \mathbf{U} \rJump^{N} = \left[ \sum^{N-1}_{j=0}
      \mathbb{U}^{j} \right] \cdot \mathbf{H} .\ 
  }
  \label{eq:Galphau7}
\end{equation}


\subsection{Update in terms of $\ddot{{u}}$}

Following a similar approach, we express the explicit update in terms of the field derivative $\ddot{{u}}$, starting from~\eqref{eq:Galphau1} and~\eqref{eq:EqGenAlpha2}. Thus, the update is 
%
\begin{equation}
  \boxed{
    \ \lJump \ddot{\mathbf{U}} \rJump^{N} = \left[ \sum^{N-1}_{j=0}
      \mathbb{U}^{j} \right] \cdot \widehat{\mathbf{H}} \ , 
  }
  \label{eq:Galphadotu1}
\end{equation}
%
where we compute the vector $\widehat{\mathbf{H}} =  \mathbb{M}^{-1} \cdot \widehat{\mathbf{L}}$ using the following definition of the right-hand side
%
\begin{align}
    \ell \left( {v} \right) = \displaystyle \frac{1}{\alpha_m}  \left[
  \left\langle  {v}  ,  {f}_{n+\alpha_f} \right\rangle - \left\langle
  {v}  ,  \ddot{{u}}_{n}  \right\rangle -  a \left(   {v}  ,  {u}_{n}
  \right) - \alpha_f \ {a}' \left(  {v}  ,  \sum_{j = 1}^{2}
  \frac{{\Delta t}^{j}}{j !} \left.{\frac{\partial^j {u}}{\partial
  t^j}}\right|_{n}  ; {u}_{n}  \right) \right].
  \label{eq:redefinitionofl}
\end{align}
%
These definitions complete the predictor/multicorrector scheme in terms of the time derivative $\ddot{{u}}$.
%
\begin{remark}
  When the update uses only the first term of the update scheme~\eqref{eq:Galphau7} or~\eqref{eq:Galphadotu1}, the update formula is similar to the explicit generalized-$\alpha$ proposed in~\cite{ HULBERT1996175}; nevertheless, our coefficients definitions are different from those used in~\cite{ HULBERT1996175}, as we discuss in the following section. Herein, we generalize the method, including the truncation error that employs higher-order terms, which allow us to predict the series convergence. 
\end{remark}

\begin{remark}
Proposed scheme does not require to update the stiffness matrix within the time increment.
\end{remark}


==> Arxiv 2/IntroductionVMC2.tex <==
\section{Introduction}
\label{section:Introduction}

Time-adaptive schemes are crucial for the efficient solution of hyperbolic partial differential equations, specifically in solid mechanics.  These highly nonlinear problems with changing boundary conditions require computationally robust adaptive numerical methods that control the time-step size to keep their cost tractable. Among several time-marching method classifications, the most conventional is the division into the explicit and implicit schemes. Some implicit schemes are unconditionally stable, allowing larger time steps, but are computationally more expensive and usually unsuitable for highly nonlinear mechanical problems~\cite{ hughes2012finite}.  Nonetheless, most time integrators for structural mechanics and deformable bodies belong to the implicit Newmark family~\cite{ Newmark1959}. Even though these implicit time-marching schemes are linearly stable, they still require numerical damping to control the detrimental impact of the poor resolution of the high-frequency modes on the problem dynamics. The engineering community continually develops implicit schemes with controlled numerical dissipation; for example,  classical methods with second-order accuracy exist, such as the Wilson-$\theta$ method~\cite{ wilson1968}, the HHT-$\alpha$ method~\cite{ Hilber1977}, the WBZ-$\alpha$~\cite{ wood1980}, the $\rho$~method~\cite{ Bazzi1982} and the $\theta_{1}$~method~\cite{ HOFF1988367, HOFF198887, HOFF198987}. In the early 90s, Chung and Hulbert proposed the generalized-$\alpha$ method, which generalizes these methods and comprises them as particular cases, to solve the hyperbolic partial differential equations that model structural dynamics problems~\cite{ chung1993time}. The generalized-$\alpha$ method controls the high-frequency dissipation while preserving accuracy in the low-frequency regions. This time-marching method successfully tackled a vast number of applications such as fluid-structure interactions~\cite{Bazilevs2006,Bazilevs2008} and finite-strain deformation~\cite{ NOELS2005358, ROSSI2016208, ScovazziIJMNE2016, BONET2015689, GIL2016146, LAVRENCIC2020107075}. Recent extensions of the method include splitting techniques~\cite{ BEHNOUDFAR2020100021} and higher-order generalized-$\alpha$ methods~\cite{ behnoudfar2019higher,BEHNOUDFAR2021113725,LOS2020109}.

Alternatively, Miranda et al.~\cite{ Miranda1989} proposed an explicit HHT-$\alpha$ method that extends the implicit HHT-$\alpha$ method, improving prior work based on the Newmark method~\cite{ Hughes1978, Hughes1978b}.  Two decades later, Hulbert and Chung~\cite{ HULBERT1996175} proposed an explicit predictor-corrector version of the generalized-$\alpha$ method, capable of controlling the numerical dissipation and maintaining the second-order accuracy, while~\cite{ Daniel2003} rewrote the classical generalized-$\alpha$ method to obtain an explicit/implicit version. Alternative explicit predictor-corrector methods in the literature are~\cite{ BONELLI2002695, Bonelli2005, Tripodi2016, lopez2020}.

Most authors use a uniform time step size to fulfil the initial CFL condition, assuming the solution behavior remains unchanged throughout the simulation, a critical weakness when dealing with nonlinear problems. The first attempts to address this limitation focused on quasi-static structural problems using continuation methods~\cite{ Thomas1973, Schmidt1978, PADOVAN1982365}. The critical time step, the maximum time-step size that ensures convergence, is related to the maximum eigenvalue of the amplification matrix. In large-scale simulations, the eigenvalue computation is extremely onerous; additionally, the stiffness matrix may change between time steps and iterations as the nonlinear process evolves. Thus, cheap convergence and error estimates are extremely valuable. Furthermore, critical time-step estimates based on eigenvalue inequalities are reliable only when the problem has a smooth response and fail when subject to sudden energy releases or impulsive loads~\cite{ Belytschko2014}. 

Other authors estimate the temporal error by comparing the discrete solution against higher-order methods; most of these methods modify Runge-Kutta integration schemes, using Butcher tables to reduce the computational cost of higher-order calculations~\cite{ Gustafsson1991, SODERLIND2006225, Butcher2016}. In structural and solid mechanics, the central difference integration with variable-step size selection was a seminal contribution in time adaptivity~\cite{ PARK1980241, UNDERWOOD1980259}, where the apparent highest frequency predicts the time-step size. Later, several authors used truncation error estimates for Newmark integrators for simple dynamics problems~\cite{ Zienkiewicz1991, Zeng1992, Wiberg1993} and extended in~\cite{ Romero2006}. Hulbert then introduced the concept of local error estimation~\cite{ HULBERT1995155} for both the explicit and implicit generalized-$\alpha$ schemes for hyperbolic partial differential equations with a focus on structural mechanics.

This paper presents an automatic time-step adaptive algorithm that uses a built-in error estimate that arises from the recursive update that the time-marching scheme uses. Our time-marching approach builds on the generalized-$\alpha$ method, allowing dissipation control in the higher frequencies while accurately approximating the low frequencies in the discrete spectrum. This method computes every update explicitly, while the system's residual corresponds to the implicit residual, ensuring the explicit dynamics track the proper nonlinear behavior of the underlying physical system. By comparing the norm of each iteration component, we evaluate the local convergence of the problem and adapt the time-step size to reach a bounded result. We apply our method to finite-strain problems to show its ability to deal with changing scenarios and non-smooth solutions. Furthermore, our scheme delivers a stable, robust, and computationally efficient formulation to solve highly nonlinear problems, preserving energy for long-integration periods even when the updating procedure uses lumping techniques.  

The paper organization follows: Section~\ref{section:insight} explains our method, while Section~\ref{section:stability} defines the method's parameters and analyses its stability. We solve the dynamics for a hyperelastic material in Section~\ref{section:nonlinear} and  detail the method's computational implementation in Section~\ref{section:Implement}. Section~\ref{section:Examples} presents theoretical and practical numerical examples; finally, we draw conclusions in Section~\ref{section:Conclusions}.

==> Arxiv 2/Nonlinear2.tex <==
\section{Hyper-elastodynamic equations}
\label{section:nonlinear}

In this section, all bold variables stands for vector-valued functions. The Hyperelasto-dynamic problem, presented in Figure \ref{fig:figure}, reads: \textit{Find the one-to-one vector field going from the reference configuration $\boldsymbol{x} \in \mathcal{B}_{0}$  to the current configuration  $\boldsymbol{X} \in \mathcal{B}$
\begin{equation}
\boldsymbol{u}\left( \boldsymbol{x} , t \right) : \mathcal{B}_{0} \to \mathcal{B} \subset \mathbb{R}^{d},
\end{equation}
that fulfills the PDE}
\begin{figure}[ht!]
\centering
{\includegraphics[height=9.25cm]{Body.pdf}}
\caption{Notation for a deformed body undergoing large strains.}
\label{fig:figure}
\end{figure}
\begin{equation}
\left\{
\begin{array}{r l l}
\rho_{0} \ddot{\boldsymbol{u}}  - \nabla_{\boldsymbol{x}} \cdot \mathcal{P}\left( \boldsymbol{u} \right) &= \rho_{0} \boldsymbol{g}  & \text{in} \ \ \mathcal{B}_{0} \times I, \\
\boldsymbol{u} \left( \boldsymbol{x} , t \right) & = \boldsymbol{u}_D \left( \boldsymbol{x} , t \right)  & \text{on}  \ \ \partial \mathcal{B}^{D}_{0} \times I,  \\
\mathcal{P}\left( \boldsymbol{u} \right) \cdot \boldsymbol{n} & =\boldsymbol{t} \left( \boldsymbol{x} , t \right) & \text{on}  \ \ \partial \mathcal{B}^{N}_{0} \times I, \\
\boldsymbol{u} \left( \boldsymbol{x} , 0 \right)   &= \boldsymbol{u}_0  & \text{on} \ \   \mathcal{B}_{0},  \\
\dot{\boldsymbol{u}}  \left( \boldsymbol{x} , 0 \right)   &= \dot{\boldsymbol{u}}_0  & \text{on} \ \   \mathcal{B}_{0},
\end{array}\right.
\label{eq:elastodynamic}
\end{equation}
where $\nabla_{\boldsymbol{x}} \left( \cdot \right)$ is the gradient in the reference configuration. In Eq. \eqref{eq:elastodynamic}, $\rho_{0}$ is the initial material density, $\partial \mathcal{B}^{D}_{0}$ and $\partial \mathcal{B}^{N}_{0}$ are the Dirichlet and Neumann part of the body boundary $\partial \mathcal{B}_{0} = \partial \mathcal{B}^{D}_{0} \cup \partial \mathcal{B}^{N}_{0}$ respectively, $\boldsymbol{g}$ is the gravity acceleration vector and $\mathcal{P}$ is the non-symmetric first Piola-Kirchhoff stress tensor defined as:
\begin{equation}
\displaystyle  \mathcal{P} = \frac{\partial \mathcal{W}}{\partial \mathcal{F}},
\label{eq:PiolaKir}
\end{equation}
with $\mathcal{F}$ gradient deformation tensor defined as,
\begin{equation}
 \mathcal{F} = \frac{\partial \boldsymbol{X}}{\partial\boldsymbol{x}} = \frac{\partial \left( \boldsymbol{x} + \boldsymbol{u} \right)}{\partial\boldsymbol{x}} = \bold{I} + \nabla_{\boldsymbol{x}} \boldsymbol{u} ,
\end{equation}
where $\bold{I}$ is the second order identity and $\mathcal{W}$ is the stored-energy function, 
\begin{equation}
\mathcal{W} = \mathcal{W}_{dev} \left(\mathcal{F} \right) + \mathcal{W}_{vol} \left(J \right),
\label{eq:storedenergy}
\end{equation}
expressed in terms of a deviatoric term which depends on the deformation gradient
\begin{equation}
\mathcal{W}_{dev} \left(\mathcal{F} \right) = \frac{\mu}{2} \left( \text{tr} \left( \mathcal{\mathcal{F}^{T} \mathcal{F}} \right) -3 \right),
\end{equation}
and a volumetric term that depends on the volumetric deformation $J = \det \mathcal{F}$
\begin{equation}
\mathcal{W}_{vol} \left(J \right) = {\lambda}   \frac{\left(J^2 -1 \right)}{4} -  \left( \frac{\lambda}{2} + \mu \right) \ln \left( J \right)  .
\end{equation}
%
The stored-energy function $\mathcal{W}$ depends on two material parameters $\lambda , \mu > 0$ which are the Lamme constants \cite{SimoandHughes1998}, while the volumetric component depends on the logarithm of the volumetric strain $J$ to prevent the element flipping.  Combining Eqs. \eqref{eq:storedenergy} and \eqref{eq:PiolaKir}, the first Piola-Kirchhoff stress tensor is obtained
\begin{equation}
\displaystyle  \mathcal{P} \left( \boldsymbol{u} \right) = \lambda \frac{J^2 - 1}{2} \mathcal{F}^{-T} + \mu \left( \mathcal{F} - \mathcal{F}^{-T} \right).
\end{equation}
%
Considering that the proposed method solves an equation system explicitly, we decided to preserve the non-symmetric stress tensor in our calculations, since it just affect the right hand side and the formulation remains in terms of a mapping given by the deformation gradient. 
%
Once the  physical problem is presented, we adjust all these set of equations to fit them in the predictor multi-corrector time-integrator we presented previously. For solving the problem \eqref{eq:elastodynamic}, we can rewrite the bi-linear form \eqref{eq:ParabolicPDEproblem} as:
\begin{equation}
a \left( \boldsymbol{v}  ,  \boldsymbol{u}  \right) = \displaystyle  \left( \nabla_{\boldsymbol{x}} \boldsymbol{v} , \mathcal{P} \left( \boldsymbol{u} \right)  \right)_{\mathcal{B}_{0}} , 
\label{eq:FuncAHyper}
\end{equation}
while the linear term is 
\begin{equation}
\displaystyle  \left\langle  \boldsymbol{v} , \boldsymbol{f} \right\rangle =  \left\langle \boldsymbol{v}  , \rho_{0} \boldsymbol{g}  \right\rangle_{\mathcal{B}_{0}}  + \left(   \boldsymbol{v}  , \boldsymbol{t} \right)_{\partial \mathcal{B}_{0}} . 
\label{eq:RHShyper}
\end{equation}
%
It is worth to note that the first term in Eq. \eqref{eq:ParabolicPDEproblem}, related with the inertia effects, is multiplied by the density as $\left\langle \boldsymbol{v} , \rho_{0} \ddot{\boldsymbol{u}}  \right\rangle$ in order to obtain a proper mass matrix. To compute a proper bilinear functional, we deploy Gateaux derivative \cite{HUGHES1978391,BatheRamm1975} on Eq. \eqref{eq:FuncAHyper} and obtain:
\begin{equation}
\overrightarrow{a} \left( \boldsymbol{v}, \lJump \boldsymbol{u} \rJump ;  \boldsymbol{u}_{n} \right)  = \displaystyle \frac{d}{d\epsilon} a \left( \boldsymbol{v} , \boldsymbol{u}_{n} + \epsilon  \lJump \boldsymbol{u} \rJump  \right) \vert_{\epsilon=0} =  \left(  \nabla_{\boldsymbol{x}} \boldsymbol{v},   \left[ \frac{\partial \mathcal{P} \left( \boldsymbol{u} \right)}{\partial \mathcal{F}} \right]_{n} \nabla_{\boldsymbol{x}} \lJump \boldsymbol{u} \rJump   \right)_{\mathcal{B}_{0}} ,
\label{eq:FuncAHypergateaux}
\end{equation}
where the tangent constitutive hyperelastic tensor is computed through the following expression
\begin{equation}
\displaystyle \frac{\partial \mathcal{P} \left( \boldsymbol{u} \right)}{\partial \mathcal{F}} =  \mathcal{F}^{-1} \left[ \lambda J^{2} \bold{I} \otimes \bold{I} + 2 \mu \left( 1 + \frac{\lambda}{2 \mu} \left( 1 - J^2 \right)\right) \boldsymbol{1}  + \left( \mathcal{P} \left( \boldsymbol{u} \right) \mathcal{F}^{T} \right) \otimes \bold{I}\right]\mathcal{F}^{-T},
\end{equation}
where $\boldsymbol{1} = \frac{1}{2} \left( \delta_{ac} \delta_{bd} + \delta_{ad} \delta_{bc}\right)$ denots a symmetric fourth-order unit tensor with $ \delta_{ij}$ being a delta Kronecker function.
%
Finally, using Eqs. \eqref{eq:FuncAHyper}, \eqref{eq:RHShyper} and \eqref{eq:FuncAHypergateaux}, the update formulas presented in \eqref{eq:Galphau7} and \eqref{eq:Galphadotu1} can be used for the time-marching calculation.


==> Arxiv 2/NonlinearVMC2.tex <==
\section{ Dynamics of hyperelasticity}
\label{section:nonlinear}

In this section, bold variables are vector-valued functions. The hyperelasto-dynamical problem that Figure~\ref{fig:figure} sketches, reads: \textit{Find the one-to-one vector field going from the reference configuration $\boldsymbol{X} \in \mathcal{B}_{0}$  to the current configuration  $\boldsymbol{x} \in \mathcal{B}$
  % 
  \begin{equation}
    \boldsymbol{u}\left( \boldsymbol{X} , t \right) : \mathcal{B}_{0} \to \mathcal{B} \subset \mathbb{R}^{d},
  \end{equation}
  that fulfills the following partial differential equations as well as the intial and boundary conditions}
% 
\begin{equation}
  \left\{
    \begin{aligned}
      \rho_{0} \ddot{\boldsymbol{u}}  - \nabla_{\boldsymbol{X}} \cdot
      \mathcal{P}\left( \boldsymbol{u} \right) &= \rho_{0}
      \boldsymbol{g}  && \text{in} \ \ \mathcal{B}_{0} \times I, \\ 
      \boldsymbol{u} \left( \boldsymbol{X} , t \right) & = \boldsymbol{u}_D
      \left( \boldsymbol{X} , t \right)  && \text{on}  \ \ \partial
      \mathcal{B}^{D}_{0} \times I,  \\ 
      \mathcal{P}\left( \boldsymbol{u} \right) \cdot \boldsymbol{n} &
      =\boldsymbol{t} \left( \boldsymbol{X} , t \right) && \text{on}  \ \
      \partial \mathcal{B}^{N}_{0} \times I, \\ 
      \boldsymbol{u} \left( \boldsymbol{X} , 0 \right)   &= \boldsymbol{u}_0
      \qquad
      \dot{\boldsymbol{u}}  \left( \boldsymbol{X} , 0 \right)   =
      \dot{\boldsymbol{u}}_0  && \text{on} \ \   \mathcal{B}_{0}, 
    \end{aligned}\right.
  \label{eq:elastodynamic}
\end{equation}%
%
\begin{figure}[ht!]
  \centering
  {\includegraphics[height=9.5cm]{Body.pdf}}
  \caption{Notation:  body undergoing large translations and deformations.}
  \label{fig:figure}
\end{figure}
%
where $\nabla_{\boldsymbol{X}} \left( \cdot \right)$ is the gradient in the reference configuration. In~\eqref{eq:elastodynamic}, $\rho_{0}$ is the initial material density, $\partial \mathcal{B}^{D}_{0}$ and $\partial \mathcal{B}^{N}_{0}$ are the Dirichlet and Neumann part of the body boundary $\partial \mathcal{B}_{0} = \partial \mathcal{B}^{D}_{0} \cup \partial \mathcal{B}^{N}_{0}$ respectively, $\boldsymbol{g}$ is the gravity's acceleration and $\mathcal{P}$ is the first Piola-Kirchhoff stress tensor defined as:
%
\begin{equation}
  \displaystyle  \mathcal{P} = \frac{\partial \,\mathsf{W}}{\partial \mathcal{F}},
  \label{eq:PiolaKir}
\end{equation}
%
with $\mathcal{F}$ being the deformation gradient tensor defined as:
%
\begin{equation}
  \mathcal{F} = \frac{\partial \boldsymbol{x}}{\partial\boldsymbol{X}}
  = \frac{\partial \left( \boldsymbol{X} + \boldsymbol{u}
    \right)}{\partial\boldsymbol{X}} = \mathcal{I} +
  \nabla_{\boldsymbol{X}} \boldsymbol{u} ,  
\end{equation}
%
where $\mathcal{I}$ is the second order identity and $\mathsf{W}$ is the stored-energy function \cite{SimoandHughes1998}, 
%
\begin{equation}
  \mathsf{W} = \mathsf{W}_{1} \left(\mathcal{F} \right) +
  \mathsf{W}_{2} \left(J \right), 
  \label{eq:storedenergy}
\end{equation}
%
that we express in terms of a  term that depends on the deformation gradient
\begin{equation}
  \mathsf{W}_{1} \left(\mathcal{F} \right) = \frac{\mu}{2} \left(
    \text{tr} \left( \mathcal{\mathcal{F}^{T} \mathcal{F}} \right) -3
  \right), 
\end{equation}
%
and another that depends on the volumetric deformation $J = \det \mathcal{F}$
%
\begin{equation}
  \mathsf{W}_{2} \left(J \right) = {\lambda}   \frac{\left(J^2 -1
    \right)}{4} -  \left( \frac{\lambda}{2} + \mu \right) \ln \left( J
  \right)  . 
\end{equation}
%
The stored-energy function $\mathsf{W}$ depends on two material parameters $\lambda , \mu > 0$, the Lamé constants,  while the second component that depends on the logarithm of the volumetric strain $J$ behaves like a penalization term that tends to prevent element flipping.  Combining~\eqref{eq:storedenergy} and~\eqref{eq:PiolaKir}, the first Piola-Kirchhoff stress tensor is
%
\begin{equation}
\displaystyle  \mathcal{P} \left( \boldsymbol{u} \right) = \lambda \frac{J^2 - 1}{2} \mathcal{F}^{-T} + \mu \left( \mathcal{F} - \mathcal{F}^{-T} \right).
\end{equation}
%
Our method solves the equation system explicitly in time; thus, we update our calculations using the non-symmetric stress tensor, which only affects the right-hand side. The formulation remains in terms of a mapping given by the deformation gradient.  Given this description of the physical problem, we adjust all these equations to fit them in our predictor multi-corrector time-marching scheme. Thus, for solving problem~\eqref{eq:elastodynamic}, we can rewrite the bi-linear form~\eqref{eq:HyperbolicPDEproblem} as:
%
\begin{equation}
  a \left( \boldsymbol{v}  ,  \boldsymbol{u}  \right) = \displaystyle
  \left( \nabla_{\boldsymbol{X}} \boldsymbol{v} , \mathcal{P} \left(
      \boldsymbol{u} \right)  \right)_{\mathcal{B}_{0}} ,  
  \label{eq:FuncAHyper}
\end{equation}
%
while the linear term is 
%
\begin{equation}
  \displaystyle  \left\langle  \boldsymbol{v} , \boldsymbol{f}
  \right\rangle =  \left\langle \boldsymbol{v}  , \rho_{0}
    \boldsymbol{g}  \right\rangle_{\mathcal{B}_{0}}  + \left(
    \boldsymbol{v}  , \boldsymbol{t} \right)_{\partial
    \mathcal{B}_{0}} .  
\label{eq:RHShyper}
\end{equation}
%
The first term in~\eqref{eq:HyperbolicPDEproblem}, the inertia term, is multiplied by the density as $\left\langle \boldsymbol{v} , \rho_{0} \ddot{\boldsymbol{u}}  \right\rangle$ in order to obtain a proper mass matrix. We obtain the bilinear functional using the Gateaux derivative~\cite{ HUGHES1978391, BatheRamm1975} on~\eqref{eq:FuncAHyper} to obtain:
%
\begin{equation}
  {a}' \left( \boldsymbol{v}, \lJump \boldsymbol{u} \rJump ;
    \boldsymbol{u}_{n} \right)  = \displaystyle \frac{d}{d\epsilon} a
  \left( \boldsymbol{v} , \boldsymbol{u}_{n} + \epsilon  \lJump
    \boldsymbol{u} \rJump  \right) \vert_{\epsilon=0} =  \left(
    \nabla_{\boldsymbol{X}} \boldsymbol{v},   \left[ \frac{\partial
        \mathcal{P} \left( \boldsymbol{u} \right)}{\partial \mathcal{F}}
    \right]_{n} \nabla_{\boldsymbol{X}} \lJump \boldsymbol{u} \rJump
  \right)_{\mathcal{B}_{0}} , 
  \label{eq:FuncAHypergateaux} 
\end{equation}
%
where the tangent constitutive hyperelastic tensor is 
%
\begin{equation}
  \displaystyle \frac{\partial \mathcal{P} \left( \boldsymbol{u}
    \right)}{\partial \mathcal{F}} =  \mathcal{F}^{-1} \left[ \lambda
    J^{2} \mathcal{I} \otimes \mathcal{I} + 2 \mu \left( 1 +
      \frac{\lambda}{2 \mu} \left( 1 - J^2 \right)\right)
    \mathfrak{1}  + \left( \mathcal{P} \left( \boldsymbol{u} \right)
      \mathcal{F}^{T} \right) \otimes \mathcal{I}\right]\mathcal{F}^{-T}, 
\end{equation}
%
where $\mathfrak{1} = \frac{1}{2} \left( \delta_{ac} \delta_{bd} + \delta_{ad} \delta_{bc}\right)$ denotes a symmetric fourth-order unit tensor with $ \delta_{ij}$ being a delta Kronecker function.  Finally, using~\eqref{eq:FuncAHyper},~\eqref{eq:RHShyper} and~\eqref{eq:FuncAHypergateaux}, we update~\eqref{eq:Galphau7} and~\eqref{eq:Galphadotu1} for the time-marching calculations.


==> Arxiv 2/StabilityVMC2.tex <==
\section{Stability and accuracy for hyperbolic problems}
\label{section:stability}

In this section, we analyze the stability analysis of our scheme following~\cite{ hughes2012finite, HULBERT1996175}. We use the spectral decomposition to simplify the set of equations to analyze
%
\begin{equation}
  \lJump  {\mathbf{U}}_{i} \rJump^{N} = \left[ \sum^{N-1}_{j=0} \left(
      -  \frac{\alpha_{f} \Delta t^{2} \beta}{\alpha_{m} }
      \omega^{2}_{i} \right)^{j} \right] \cdot
  \widetilde{\mathbf{H}}_{i}, 
\end{equation}
%
where $\omega_{i}$ are the eigenvalues of the system
%
\begin{equation}
  \left(\mathbb{M}^{-1} \mathbb{K} - \omega^{2}_{i}  \mathbb{I} \right)
  \Psi_{i} = \mathbf{0}, 
  \label{eq:freq}
\end{equation}
%
that represent the frequency of mode $i$ for the base vector $\Psi_{i}$. Furthermore, we use a compact notation for the sum term:
%
\begin{equation}
  \left[{P^{N}_{k}} \right]_{i} =  \sum^{N-1}_{j=k} \left( -
    \frac{\alpha_{f} \Delta t^{2} \beta}{\alpha_{m} } \omega^{2}_{i}
  \right)^{j} .
  \label{eq:modaldecomposition}
\end{equation}
%
In what follows, we spectrally decompose the matrix in~\eqref{eq:modaldecomposition}. This decomposition allows us to obtain a set of parameters that control the method's dissipation and stability region.

\subsection{Accuracy analysis}

Herein, before analyzing the method's stability behavior, we study its order of accuracy.  We seek to deliver second-order accuracy in time; therefore, we define the parameter $\gamma$ as follows
%
\begin{thm} \label{thm:3o}
  We obtain a scheme with second-order accuracy in time by setting
  %
  \begin{equation} \label{eq:3ov1}
    \gamma=\frac{1}{2}-\alpha_{f}+\alpha_m.
  \end{equation}
\end{thm}
\begin{proof}
  We consider~\eqref{eq:EqGenAlpha2} and the displacement update formula~\eqref{eq:Galphau7}, and perform algebraic substitutions; then, the equation system at each time step $n+1$ in terms of a known right-hand side becomes
  % 
  \begin{equation}
    \mathbb{A} \mathbf{X}_{n+1} = \mathbb{B} \mathbf{X}_{n} + \mathbf{F}^{\sharp}_{n+\alpha_f},
  \end{equation}
  %
  where the matrices and vectors are
  \begin{equation}
    \begin{aligned}\mathbb{A}&=
      \begin{bmatrix}
	1 & 0 & -\beta \\
	0 & 1 & -\gamma \\
	1& 0 & 0 \\
      \end{bmatrix},
      &
      \mathbb{B}&=
      \begin{bmatrix}
	1 & 1 & \displaystyle \frac{1}{2}-\beta \\
	0 & 1 & \displaystyle 1-\gamma \\
	\displaystyle   1 + \frac{1}{\alpha_f}   \left[{P^{N}_{1}}
        \right]_{i} & \displaystyle \left[{P^{N-1}_{0}} \right]_{i} &
        \displaystyle \left( \frac{1}{2} - \frac{\beta }{\alpha_m }
        \right) \left[{P^{N-1}_{0}} \right]_{i} 
      \end{bmatrix},\\
      \mathbf{X}_{n}&=
      \begin{bmatrix}
	\mathbf{U}_{n}  \\
	\Delta t \ \dot{\mathbf{U}}_{n}  \\
	\Delta t^2 \ddot{\mathbf{U}}_{n}\\ 
      \end{bmatrix}, &
      \mathbf{F}^{\sharp}_{n+\alpha_f} &=
      \begin{bmatrix}		
	0 \\
	0 \\
	\displaystyle \frac{\beta \Delta t^2}{\alpha_m}
        \left[{P^{N-1}_{0}} \right]_{i} \left[\mathbb{M}^{-1}
          \mathbf{F}_{n+\alpha_f}  \right]_{i}  
      \end{bmatrix}.
    \end{aligned}
  \end{equation}
  % 
  We update the matrices using the acceleration update formula~\eqref{eq:Galphadotu1}, 
  %
  \begin{equation}
    \begin{aligned}\mathbb{A}&=
      \begin{bmatrix}
	1 & 0 & -\beta \\
	0 & 1 & -\gamma \\
	0& 0 & 1 \\
      \end{bmatrix},\qquad\qquad
      \mathbb{B}=
      \begin{bmatrix}
	1 & 1 & \displaystyle \frac{1}{2}-\beta \\
	0 & 1 & \displaystyle 1-\gamma \\
	\displaystyle   \frac{1}{\alpha_f  \beta } \left[{P^{N}_{1}}
        \right]_{i} & \displaystyle   \frac{1}{ \beta}
        \left[{P^{N}_{1}} \right]_{i} & \displaystyle   1 -
        \frac{1}{\alpha_m} \left[{P^{N-1}_{0}} \right]_{i} +
        \frac{1}{2 \beta} \left[{P^{N}_{1}} \right]_{i}  
      \end{bmatrix}\\
           \mathbf{F}^{\sharp}_{n+\alpha_f} &=
      \begin{bmatrix}		
	0 \\
	0 \\
	\displaystyle \frac{1}{\alpha_m} \left[{P^{N-1}_{0}}
        \right]_{i} \left[\mathbb{M}^{-1}  \mathbf{F}_{n+\alpha_f}
        \right]_{i}  
      \end{bmatrix}.
    \end{aligned}
  \end{equation}
  % 
  The amplification matrix  $\mathbb{G}$ for a hyperbolic problem is
  %
  \begin{equation} \label{eq:ampm}
    \mathbb{G}=\mathbb{A}^{-1}\mathbb{B}.
  \end{equation}
  %
  For an arbitrary $3\times 3$ invertible matrix, we can state~\cite{ hughes2012finite}:
  %
  \begin{equation} \label{eq:a40}
    \mathbb{G}_0 \bold{U}_{n+1} - \mathbb{G}_1 \bold{U}_n +
    \mathbb{G}_2 \bold{U}_{n-1} - \mathbb{G}_3 \bold{U}_{n-2} = 0, 
  \end{equation}
  %
  where the coefficients $\mathbb{G}_i$ for $i=1,2,3$ are the amplification matrix invariants; that is, $\mathbb{G}_0 = 1$, $\mathbb{G}_1 $ is the trace of $\mathbb{G}$, $\mathbb{G}_2$ is the sum of principal minors of $\mathbb{G}$, and $\mathbb{G}_3$ is the determinant of $\mathbb{G}$. Using a Taylor expansion analogous to the one in~\eqref{eq:EqGenAlpha2}, we obtain
  %
  \begin{equation} \label{eq:Taypar}
    \begin{aligned}
      \bold{U}_{n+1} & = \bold{U}_n + \Delta t \dot{\bold{U}}_n +
      \dfrac{\Delta t^2}{2} \ddot{\bold{U}}_n+\mathcal{O}(\tau^3), \\ 
      \bold{U}_{n-1} & = \bold{U}_n - \Delta t
      \dot{\bold{U}}_n+\dfrac{\Delta t^2}{2}
      \ddot{\bold{U}}_n+\mathcal{O}(\tau^3), \\ 
      \bold{U}_{n-2} & = \bold{U}_n - 2 \Delta t \dot{\bold{U}}_n +
      4\frac{\Delta t^2}{2} \ddot{\bold{U}}_n +\mathcal{O}(\tau^3). 
    \end{aligned}
  \end{equation}
  % 
  Then, substituting~\eqref{eq:Taypar} into~\eqref{eq:a40} and setting the sum limit $N=2$ in~\eqref{eq:modaldecomposition}, we obtain
  %
  \begin{multline}
    \frac{\left[{P^{1}_{1}} \right]^2 \left(4 \beta
        (\alpha_f-\alpha_m)+\alpha_m (-4 \alpha_f (\gamma-1)+6
        \gamma-5)\right)}{4 \beta^2}\bold{U}_n\\
    + 
    \left[{P^{1}_{1}} \right]^2 \alpha_m \Delta t
    \left(\frac{\alpha_f (3 \gamma-2) }{3 \beta^2}-\frac{7 \gamma
      }{6 \beta^2}+\frac{3 }{4 \beta^2}-\frac{\alpha_f }{\beta
        \alpha_m}+\frac{1}{\beta}\right)\dot{\bold{U}}_n \\+  
    \dfrac{\left[{P^{1}_{1}} \right] \Delta t}{\beta}
    \left(-\alpha_f -\gamma +\alpha_m
      +\frac{1}{2}\right)\ddot{\bold{U}}_n = 0 . 
  \end{multline}
  % 
  Next, we obtain second-order accuracy by canceling the third term in the last equation; thus, we set
  %
  \begin{equation}
    \gamma=\frac{1}{2}-\alpha_{f}+\alpha_m.
  \end{equation}
  %
  This completes our proof.
  %
  \begin{remark}
    %
    For values of $N>2$, we can follow a similar approach as the higher-order terms of $\left[{P^{N}_{1}} \right]$, noting that these terms do not affect the accuracy order.  
    %
  \end{remark}
\end{proof}
%
\subsection{Stability analysis and CFL conditions}\label{sec:anal}

We can control the solution stability by bounding the spectral radius of the method; that is, the absolute value of the eigenvalues of the amplification matrix must be bounded by one. First, we calculate the eigenvalues of the amplification matrix for hyperbolic problems in~\eqref{eq:ampm} for the case $ \Delta t^{2}\omega_{i}^{2} \to 0$ as:
%
\begin{equation}\label{eq:t0}
  \lambda_1=\lambda_2=1,\qquad \lambda_3=\frac{\alpha_m-1}{\alpha_m}.
\end{equation}
% 
The bounding  $\lambda_3$ in~\eqref{eq:t0} implies that $ {\alpha_m}\geq \frac{1}{2} $. 

We derive our method's CFL condition~\cite{ Courant56}. The implicit generalized-$\alpha$ method proposed in~\cite{ chung1993time, behnoudfar2019higher} are unconditionally stable. For these methods we study their high-frequency eigenvalues in the limit where $\Theta:= \Delta t^{2}\omega_{i}^{2} \to \infty$ where $\omega_{i}$ denotes the corresponding eigenvalue of the spatial discretization (eigenvalue of $\mathbb{M}^{-1}\mathbb{K}$). Thus, to guarantee unconditional stability, we set the parameters such that the eigenvalues are equal to a constant $\rho_\infty \in [0,1]$, which controls the numerical dissipation.

In our predictor multi-corrector method, we need to find a stable region due to its conditional behavior. Therefore, we only consider two of the roots of the characteristic polynomial as principal roots, while the third is spurious.  We maximize high-frequency dissipation by enforcing the principal roots to remain complex conjugate except in the high-frequency limit; the principal roots bifurcate only in the high-frequency limit.  Here, we denote the high-frequency limit as the critical stability limit, $\Omega_s$. Root bifurcation decreases the high-frequency dissipation; thus, our method's two limits of concern are $\Omega_s$ and the bifurcation limit $\Omega_b$.  The characteristic equation of the amplification matrix reads
%
\begin{equation}\label{eq:char}
  \sum_{j=0}^{3}\left(\tilde{a}^j+\tilde{y}^j \Theta^2\right)\lambda^{(3-j)}=0,
\end{equation}
%
where $\tilde{a}$ and $\tilde{y}$ depend on parameters such as $\gamma$ and $\beta$. The characteristic polynomial of $\mathbb{G}$ in~\eqref{eq:ampm} is
%
\begin{multline}\label{eq:charG}
  -\lambda^3+\lambda^2 \left(-\frac{\alpha_f^2 \left[{P^{1}_{1}}
      \right]}{\beta}+\frac{\alpha_f \alpha_m \left[{P^{1}_{1}}
      \right]}{\beta}+\frac{\alpha_f \left[{P^{1}_{1}}
      \right]}{\beta}-\frac{\alpha_f  \left[{P^{1}_{1}}
      \right]}{\alpha_m}-\frac{1}{\alpha_m}+\left[{P^{1}_{1}}
    \right]+3\right)\\ 
  +\lambda \left(\frac{2 \alpha_f^2 \left[{P^{1}_{1}}
      \right]}{\beta}-\frac{2 \alpha_f \alpha_m \left[{P^{1}_{1}}
      \right]}{\beta}-\frac{2 \alpha_f \left[{P^{1}_{1}}
      \right]}{\beta}+ 
      \frac{\alpha_m \left[{P^{1}_{1}}
      \right]}{\beta}+\frac{\left[{P^{1}_{1}} \right]}{\beta}+\frac{2
      \alpha_f \left[{P^{1}_{1}}
      \right]}{\alpha_m}+\frac{2}{\alpha_m}-2 \left[{P^{1}_{1}}
    \right]-3\right)\\ 
  -\frac{\alpha_f^2 \left[{P^{1}_{1}} \right]}{\beta}+\frac{\alpha_f
    \alpha_m \left[{P^{1}_{1}} \right]}{\beta}+\frac{\alpha_f
    \left[{P^{1}_{1}} \right]}{\beta}-\frac{\alpha_m \left[{P^{1}_{1}}
    \right]}{\beta}-\frac{\alpha_f \left[{P^{1}_{1}}
    \right]}{\alpha_m}-\frac{1}{\alpha_m}+\left[{P^{1}_{1}} \right]+1=0 
\end{multline}
% 
We set two eigenvalues to $\rho_{b}$ and one becomes $\rho_{s}$. Thus, we rewrite the characteristic polynomial~\eqref{eq:char} as
%
\begin{equation}\label{eq:root}
\left(\lambda^2+\rho_{b}^2+2\lambda\rho_{b}\right)\left(\lambda+\rho_{s}\right)=0,
\end{equation}
%
where $\lambda$, $\rho_{b}$, and $\rho_{s}$ are the eigenvalues, and user-defined values, respectively.  The bifurcation limit $\Omega_{b}$ shows when the largest eigenvalue decreases from one and converges to the user-defined parameters $\rho_{b}$. Following a similar argument to~\cite{ HULBERT1996175}, having all three roots with real values at the bifurcation limit, we equate~\eqref{eq:root} and~\eqref{eq:char} and solve for the parameters $\alpha_m, \left[ P^{1}_{1} \right] ,\,\beta$. Then, we obtain two parameters
%
\begin{align}\label{eq:par}
\alpha_m=&\frac{-{\rho_b} {\rho_s}+{\rho_s}+2}{{\rho_b} {\rho_s}+{\rho_b}+{\rho_s}+1},
\end{align}
%
and
%
\begin{align}\label{eq:parbeta}
  \beta = \frac{
  \splitfrac{
  \alpha_f \left(\rho_b+1\right)
  \left\{\alpha_f \left( \rho_b+1\right)
  \left(\rho_s+1\right) \left[\left(\rho_b-1\right)
  \rho_s-2\right]
  -\rho_b^2
  \rho_s+2 \rho_b \left(\rho_s^2+\rho_s-1\right)-2 \rho_s^2-7
  \rho_s-6\right\}
  } { 
  + 2 \rho_b^2 \rho_s+\rho_b \left(\rho_s^2+2 \rho_s-3\right)-\rho_s^2-4 
  \rho_s-5 } }
  {\left(\rho_b+1\right)^2 \left(\rho_s+1\right)
  \left[\alpha_f (\rho_b+1) (\rho_s+1)+(\rho_b-1) \rho_s-2\right]
  }.  
\end{align}
%
We optimize the method's dissipation control using the available parametrization. We set $\rho_b=\rho_s$ and, for the sake of brevity, we omit many algebraic manipulations.  Therefore, our method reduces to a one-parameter technique with the following bifurcation limit $\Omega_{b}$
%
\begin{equation}
  \sum_{k=1}^{N}\left(\dfrac{\beta}{\alpha_m} \Omega_b\right)^k
  =-\frac{(\rho_{b}+1) \left[\alpha_f^2 (\rho_{b}-2) (\rho_{b}+1)^2+\alpha_f
      \left(-3 \rho_{b}^2+3 \rho_{b}+6\right)+3 \rho_{b}-5\right]}{\alpha_f
    \rho_{b}+\alpha_f+\rho_{b}-2}. 
\end{equation} 
%
We determine the stability region by finding the conditions under which the spectral radius grows to one after its bifurcation. For this, we propose the following
%
\begin{equation}\label{eq:stab}
  \sum_{k=1}^{N}\left(\dfrac{\beta}{\alpha_m} \Omega_s\right)^k
  =-\frac{\beta (4-8 \alpha_m)}
  {4 \beta (\alpha_f-\alpha_m)+2 \alpha_m
    \left[2\alpha_f- (\alpha_f-\alpha_m-1)+\alpha_m\right]+\alpha_m}. 
\end{equation}
%
Letting $N=1$, we substitute the definitions~\eqref{eq:par} into~\eqref{eq:stab} to obtain
%
\begin{equation}\label{eq:stabf}
  \Omega_s=-\frac{12 (\rho_{b}-2) (\rho_{b}+1)}{\rho_{b}^2-5 \rho_{b}+10}.
\end{equation}
%
\begin{remark}
  Following~\cite{ HULBERT1996175,  behnoudfar2018variationally, BEHNOUDFAR2021113656} and considering~\eqref{eq:stabf}, $\alpha_{f}$ is a free parameter with respect to spectral radius; thus, we obtain the optimal combination of low- and high-frequency dissipation by setting  $\alpha_{f}=0$ and letting the remaining parameters be:
  %
  \begin{equation}
    \boxed{
      \begin{aligned}
        \alpha_m&= \frac{2-\rho_{b}}{\rho_{b}+1},\\
        \beta&= \frac{3 \rho_{b}-5}{(\rho_{b}-2) (\rho_{b}+1)^2},\\
        \Omega_b&= \frac{-3 \rho_{b}^2+2 \rho_{b}+5}{\rho_{b}-2}.
      \end{aligned}
    }
    \label{eq:Galphaparametersprev}
  \end{equation}
\end{remark}
\begin{remark}
  Setting $\rho_{b}(=\rho_b=\rho_s)=1$ leads to the largest stability region $\Omega_s=4$ which is equivalent to the second-order central difference method~\cite{ hairer2010solving}. This stability region imposes the following CFL condition $\Delta t^2\leq\dfrac{4}{\omega_{i}}$ on our method.
\end{remark}
%
We perform a similar analysis for higher-order methods, that is, $N>1$. Herein, we analyze the case of choosing $N=2$. We first determine the stability region as
%
\begin{equation}
  \Omega_s= \dfrac{\alpha_m-\alpha_m \sqrt{1-\dfrac{4\beta (4-8
        \alpha_m)}{4 \beta (\alpha_f-\alpha_m)+2 \alpha_m (2\alpha_f-
        (\alpha_f-\alpha_m-1)+\alpha_m)+\alpha_m}}}{2 \beta}. 
\end{equation}
%
Here, we cannot set $\alpha_f=0$; then, we have
%
\begin{equation}
  \boxed{
    \begin{aligned}
      \alpha_m&= \frac{2-\rho_{b}}{\rho_{b}+1},\\
      \beta&=\frac{\alpha_f^2 (\rho_{b}-2) (\rho_{b}+1)^2+\alpha_f \left(-3 \rho_{b}^2+3 \rho_{b}+6\right)+3 \rho_{b}-5}{(\rho_{b}+1)^2 (\alpha_f \rho_{b}+\alpha_f+\rho_{b}-2)},\\
      \alpha_f&=\dfrac{4}{1+4\rho_{b}}
    \end{aligned}
  }
  \label{eq:Galphaparameters}
\end{equation}
%

==> Arxiv 2/abstractVMC2.tex <==
We propose a time-adaptive predictor/multi-corrector method to solve hyperbolic partial differential equations, based on the generalized-$\alpha$ scheme that provides user-control on the numerical dissipation and second-order accuracy in time. Our time adaptivity uses an error estimation that exploits the recursive structure of the variable updates. The predictor/multicorrector method explicitly updates the equation system but computes the residual of the system implicitly. We analyze the method's stability and describe how to determine the parameters that ensure high-frequency dissipation and accurate low-frequency approximation. Subsequently, we solve a linear wave equation, followed by non-linear finite strain deformation problems with different boundary conditions. Thus, our method is a straightforward, stable and computationally efficient approach to simulate real-world engineering problems. Finally, to show the performance of our method, we provide several numerical examples in two and three dimensions.  These challenging tests demonstrate that our predictor/multicorrector scheme dynamically adapts to sudden energy releases in the system, capturing impacts and boundary shocks. The method efficiently and stably solves dynamic equations with consistent and under-integrated mass matrices conserving the linear and angular momenta as well as the system's energy for long-integration times.

\textbf{Keywords:} Time - adaptivity, Stability, Finite-strain, Dissipation control, Hyperbolic equations.



==> Arxiv 2/commands.tex <==
\newfont{\tenbfsl}{cmbxti9 scaled 1200}
\newfont{\tenbbb}{msbm10}
\newfont{\svnbbb}{msbm8}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Fractions
\newcommand{\half}{\textstyle{\frac{1}{2}}}
\newcommand{\third}{\textstyle{\frac{1}{3}}}
\newcommand{\fourth}{\textstyle{\frac{1}{4}}}

% Fonts
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\br}[1]{\boldsymbol{\mathrm{{#1}}}}
\newcommand{\bi}[1]{\boldsymbol{\mathit{{#1}}}}
\newcommand{\cl}[1]{\mathcal{#1}}
\newcommand{\mt}[1]{\mathit{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\fk}[1]{\mathfrak{#1}}
\newcommand{\ms}[1]{\mathds{#1}}
% \newcommand{\bb}[1]{\mbox{\tenbbb {#1}\/}}
% \newcommand{\sbb}[1]{\mbox{\svnbbb {#1}\/}}

\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\green}[1]{{\color{green} #1}}

% Indentity tensor
% \newcommand{\id}{\mbox{\tenbfsl 1\/}}
\newcommand{\id}{\bs{1}}

\newcommand{\sbet}{\stackrel{!}{=}}

\newcommand{\norm}[2]{\left\lVert {#1} \right\rVert_{#2}}
\newcommand{\lrang}[2]{\left\langle {#1}, {#2} \right\rangle}
\newcommand{\lrpar}[2]{\left( {#1}, {#2} \right)}
\newcommand{\lrrec}[2]{\left[ {#1}, {#2} \right]}
\newcommand{\lrcha}[2]{\left\{ {#1}, {#2} \right\}}
\newcommand{\jump}[1]{\llbracket {#1} \rrbracket}
\newcommand{\surp}[1]{\{\!\!\{ {#1} \}\!\!\}}
\newcommand{\bpnt}[1]{\rrbracket {#1} \llbracket}
\newcommand{\jumpl}{\llbracket}
\newcommand{\surpl}{\{\!\!\{}
\newcommand{\bpntl}{\rrbracket}
\newcommand{\jumpr}{\rrbracket}
\newcommand{\surpr}{\}\!\!\}}
\newcommand{\bpntr}{\llbracket}

\newcommand{\fr}[2]{{\textstyle{\frac{{#1}}{{#2}}}}}

% Differentials
\newcommand{\di}{\,\mathrm{d}}
\newcommand{\dvr}{\,\mathrm{d}V}
\newcommand{\dar}{\,\mathrm{d}A}
\newcommand{\dsr}{\,\mathrm{d}S}
\newcommand{\dv}{\,\mathrm{d}v}
\newcommand{\da}{\,\mathrm{d}a}
\newcommand{\ds}{\,\mathrm{d}\sigma}
\newcommand{\dx}{\,\mathrm{d}x}

% Parts
\newcommand{\bdy}{\cl{B}}
\newcommand{\dbdy}{\partial\cl{B}}
\newcommand{\prt}{\cl{P}}
\newcommand{\dprt}{\partial\cl{P}}
\newcommand{\srf}{\cl{S}}
\newcommand{\dsrf}{\partial\cl{S}}
\newcommand{\ddsrf}{\partial^2\cl{S}}
\newcommand{\edg}{\cl{C}}
\newcommand{\dedg}{\partial\cl{C}}
\newcommand{\pnt}{\cl{O}}

% Integrals
\newcommand{\intP}{\int\limits_{\prt}}
\newcommand{\intdP}{\int\limits_{\dprt}}
\newcommand{\intS}{\int\limits_{\srf}}
\newcommand{\intdS}{\int\limits_{\partial\srf}}
\newcommand{\intC}{\int\limits_{\edg}}

% Spacing
\newcommand{\vs}{\mskip2mu}
\newcommand{\vvs}{\mskip1mu}

% Algebraic tensor operations
\newcommand{\trans}{\scriptscriptstyle\mskip-1mu\top\mskip-2mu}
\newcommand{\axial}{\scriptscriptstyle\mskip-1mu\times\mskip-2mu}
\newcommand{\sperp}{\scriptscriptstyle\mskip-2mu\perp\mskip-2mu}
\newcommand{\trbck}{\mathbin{\rotatebox[origin=c]{-90}{$\trans$}}}
\newcommand{\trfrw}{\mathbin{\rotatebox[origin=c]{90}{$\trans$}}}
\newcommand{\tr}{\mathrm{tr}\mskip2mu}
\newcommand{\sym}{\mathrm{sym}\mskip2mu}
\newcommand{\skw}{\mathrm{skw}\mskip2mu}
\newcommand{\ax}{\mathrm{ax}\mskip2mu}
\newcommand{\dotr}{\mbox{${\cdot}$}}

% Differential tensor operations
\newcommand{\Grad}{\mathrm{Grad}\mskip2mu}
\newcommand{\Div}{\mathrm{Div}\mskip2mu}
\newcommand{\Curl}{\mathrm{curl}\mskip2mu}
\newcommand{\Grads}{\Grad_{\mskip-2mu\scriptscriptstyle\cl{S}}}
\newcommand{\Divs}{\Div_{\mskip-6mu\scriptscriptstyle\cl{S}}}

% Partial derivatives
\newcommand{\pards}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\lpards}[2]{\partial{#1}/\partial{#2}}
\newcommand{\dd}[2]{\frac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}
\newcommand{\ldd}[2]{\mathrm{d}{#1}/\mathrm{d}{#2}}

% Space and time
\newcommand{\xt}{(\bs{x},t)}

% To fix spacing in integrals in multiple lines
\newcommand{\intvspace}{\vphantom{\int\limits_{\dprt\dbdy_\tau}}}
\newcommand{\sumvspace}{\vphantom{\sum_{\alpha=1}^n}}

% Theorems
\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{prp}{Proposition}
\newtheorem{ass}{Assumption}
\newtheorem{pst}{Postulate}
\theoremstyle{remark}
\newtheorem{rmk}{Remark}
\newtheorem{pry}{Property}
\newtheorem{scn}{Setting}
\theoremstyle{definition}
\newtheorem{set}{Definition}

%------------------------------------------------------------------------------%

% Synopsis
\newcounter{syn}[section] \setcounter{syn}{0}
\renewcommand{\thesyn}{\arabic{section}.\arabic{syn}}
\newenvironment{syn}[2][]{%
\refstepcounter{syn}%
\ifstrempty{#1}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,rounded corners,fill=Violet!20,draw= Violet!50, double= Violet!50]
% \tikz[baseline=(current bounding box.east),outer sep=0pt]
% \node[anchor=east,rectangle,fill=blue!20]
{\strut Synopsis~\thesyn};}}
}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,rounded corners,fill=Violet!20,draw= Violet!50, double= Violet!50]
% \tikz[baseline=(current bounding box.east),outer sep=0pt]
% \node[anchor=east,rectangle,fill=blue!20]
{\strut Synopsis~\thesyn:~#1};}}%
}%
\mdfsetup{innertopmargin=10pt,linecolor=Violet!50,backgroundcolor=Violet!5,%
% \mdfsetup{innertopmargin=10pt,linecolor=blue!20,%
linewidth=2pt,topline=true,%
frametitleaboveskip=\dimexpr-\ht\strutbox\relax
}
\begin{mdframed}[]\relax%
\label{#2}}{\end{mdframed}}

%------------------------------------------------------------------------------%

% contractions
\newcommand{\twovdots}{\mskip+2mu\colon\mskip-2mu}
\makeatletter
\def\threevdots{\mskip+4mu\vbox{\baselineskip2.25\p@ \lineskiplimit\z@
  \kern4.9\p@\hbox{.}\hbox{.}\hbox{.}}\mskip+3.8mu}
\makeatother
\newcommand{\fourvdots}{\mskip+2mu\colon\mskip-7mu\colon\mskip-2mu}

% Projectors

\newcommand{\Prj}[1]{\br{P}_{\mskip-6mu{#1}}}

% other symbols
\newcommand{\xis}{\xi_{\scriptscriptstyle\cl{S}}}
\newcommand{\xiss}{\tensor*[^2]{\xi}{^\alpha_{\scriptscriptstyle\cl{S}}}}
\newcommand{\xisss}{\tensor*[^3]{\xi}{^\alpha_{\scriptscriptstyle\cl{S}}}}
\newcommand{\xids}{\xi_{\scriptscriptstyle\partial\cl{S}}}
\newcommand{\xic}{\xi_{\scriptscriptstyle\cl{C}}}
\newcommand{\xiccn}{\tensor*[^2_n]{\xi}{^\alpha_{\scriptscriptstyle\cl{C}}}}
\newcommand{\xiccnu}{\tensor*[^2_\nu]{\xi}{^\alpha_{\scriptscriptstyle\cl{C}}}}
\newcommand{\xidc}{\xi_{\scriptscriptstyle\partial\cl{C}}}
\newcommand{\xio}{\xi_{\scriptscriptstyle\cl{O}}}
\newcommand{\bsvarpis}{\bs{\varpi}_{\mskip-2mu\scriptscriptstyle\cl{S}}}
\newcommand{\bsvarpids}{\bs{\varpi}_{\mskip-2mu\scriptscriptstyle\partial\cl{S}}}
\newcommand{\bsvarpic}{\bs{\varpi}_{\mskip-2mu\scriptscriptstyle\cl{C}}}
\newcommand{\sigmas}{{\sigma_{\mskip-1mu\scriptscriptstyle\cl{S}}}}
\newcommand{\bsvarsigmas}{{\bs{\varsigma}_{\mskip-1mu\scriptscriptstyle\cl{S}}}}

\newcommand{\rvecdc}{{\bs{r}_{\mskip-1mu\scriptscriptstyle\partial\cl{C}}}}
\newcommand{\rveco}{{\bs{r}_{\mskip-1mu\scriptscriptstyle\cl{O}}}}

% Clebsch--Gordan coefficients
\newcommand{\ellcg}[2]{\tensor*[^{#1}]{\ell}{_{#2}}}

\newcommand{\bsts}{\bs{t}_{\scriptscriptstyle\cl{S}}}
\newcommand{\bstss}{\tensor*[^2]{\bs{t}}{_{\scriptscriptstyle\cl{S}}}}
\newcommand{\bstsss}{\tensor*[^3]{\bs{t}}{_{\scriptscriptstyle\cl{S}}}}
\newcommand{\bstds}{\bs{t}_{\scriptscriptstyle\partial\cl{S}}}
\newcommand{\bstc}{\bs{t}_{\scriptscriptstyle\cl{C}}}
\newcommand{\bstccn}{\tensor*[^2_n]{\bs{t}}{_{\scriptscriptstyle\cl{C}}}}
\newcommand{\bstccnu}{\tensor*[^2_\nu]{\bs{t}}{_{\scriptscriptstyle\cl{C}}}}
\newcommand{\bstdc}{\bs{t}_{\scriptscriptstyle\partial\cl{C}}}
\newcommand{\bsto}{\bs{t}_{\scriptscriptstyle\cl{O}}}
\newcommand{\bsms}{\bs{m}_{\scriptscriptstyle\cl{S}}}
\newcommand{\bsmds}{\bs{m}_{\scriptscriptstyle\partial\cl{S}}}
\newcommand{\bsmc}{\bs{m}_{\scriptscriptstyle\cl{C}}}

\newcommand{\bstsast}{\bs{t}_{\scriptscriptstyle\cl{S}^{\ast}}}
\newcommand{\bstcast}{\bs{t}_{\scriptscriptstyle\cl{C}^{\ast}}}
\newcommand{\bsmsast}{\bs{m}_{\scriptscriptstyle\cl{S}^{\ast}}}
\newcommand{\bsmcast}{\bs{m}_{\scriptscriptstyle\cl{C}^{\ast}}}
\newcommand{\xisast}{\xi_{\scriptscriptstyle\cl{S}^{\ast}}}
\newcommand{\xicast}{\xi_{\scriptscriptstyle\cl{C}^{\ast}}}
\newcommand{\bsvarpisast}{\bs{\varpi}_{\mskip-2mu\scriptscriptstyle\cl{S}^{\ast}}}
\newcommand{\bsvarpicast}{\bs{\varpi}_{\mskip-2mu\scriptscriptstyle\cl{C}^{\ast}}}

\newcommand{\kappas}{\kappa_{\scriptscriptstyle\cl{S}}}
\newcommand{\kappads}{\kappa_{\scriptscriptstyle\partial\cl{S}}}
\newcommand{\kappao}{\kappa_{\scriptscriptstyle\cl{O}}}
\newcommand{\bskappas}{\bs{\kappa}_{\scriptscriptstyle\cl{S}}}
\newcommand{\bskappads}{\bs{\kappa}_{\scriptscriptstyle\partial\cl{S}}}

\newcommand{\migd}[2]{\tensor[^{#2}]{\mathrm{d}}{_{#1}}}
\newcommand{\migp}[2]{\tensor[^{#2}]{\partial}{_{#1}}}
\newcommand{\vlat}{\upsilon_{\scriptscriptstyle\partial\cl{S}}}
\newcommand{\vsurf}{\upsilon_{\scriptscriptstyle\cl{S}}}


==> Nonlinear2.tex <==
\section{Hyper-elastodynamic equations}
\label{section:nonlinear}

In this section, all bold variables stands for vector-valued functions. The Hyperelasto-dynamic problem, presented in Figure \ref{fig:figure}, reads: \textit{Find the one-to-one vector field going from the reference configuration $\boldsymbol{x} \in \mathcal{B}_{0}$  to the current configuration  $\boldsymbol{X} \in \mathcal{B}$
\begin{equation}
\boldsymbol{u}\left( \boldsymbol{x} , t \right) : \mathcal{B}_{0} \to \mathcal{B} \subset \mathbb{R}^{d},
\end{equation}
that fulfills the PDE}
\begin{figure}[ht!]
\centering
{\includegraphics[height=9.25cm]{Body.pdf}}
\caption{Notation for a deformed body undergoing large strains.}
\label{fig:figure}
\end{figure}
\begin{equation}
\left\{
\begin{array}{r l l}
\rho_{0} \ddot{\boldsymbol{u}}  - \nabla_{\boldsymbol{x}} \cdot \mathcal{P}\left( \boldsymbol{u} \right) &= \rho_{0} \boldsymbol{g}  & \text{in} \ \ \mathcal{B}_{0} \times I, \\
\boldsymbol{u} \left( \boldsymbol{x} , t \right) & = \boldsymbol{u}_D \left( \boldsymbol{x} , t \right)  & \text{on}  \ \ \partial \mathcal{B}^{D}_{0} \times I,  \\
\mathcal{P}\left( \boldsymbol{u} \right) \cdot \boldsymbol{n} & =\boldsymbol{t} \left( \boldsymbol{x} , t \right) & \text{on}  \ \ \partial \mathcal{B}^{N}_{0} \times I, \\
\boldsymbol{u} \left( \boldsymbol{x} , 0 \right)   &= \boldsymbol{u}_0  & \text{on} \ \   \mathcal{B}_{0},  \\
\dot{\boldsymbol{u}}  \left( \boldsymbol{x} , 0 \right)   &= \dot{\boldsymbol{u}}_0  & \text{on} \ \   \mathcal{B}_{0},
\end{array}\right.
\label{eq:elastodynamic}
\end{equation}
where $\nabla_{\boldsymbol{x}} \left( \cdot \right)$ is the gradient in the reference configuration. In Eq. \eqref{eq:elastodynamic}, $\rho_{0}$ is the initial material density, $\partial \mathcal{B}^{D}_{0}$ and $\partial \mathcal{B}^{N}_{0}$ are the Dirichlet and Neumann part of the body boundary $\partial \mathcal{B}_{0} = \partial \mathcal{B}^{D}_{0} \cup \partial \mathcal{B}^{N}_{0}$ respectively, $\boldsymbol{g}$ is the gravity acceleration vector and $\mathcal{P}$ is the non-symmetric first Piola-Kirchhoff stress tensor defined as:
\begin{equation}
\displaystyle  \mathcal{P} = \frac{\partial \mathcal{W}}{\partial \mathcal{F}},
\label{eq:PiolaKir}
\end{equation}
with $\mathcal{F}$ gradient deformation tensor defined as,
\begin{equation}
 \mathcal{F} = \frac{\partial \boldsymbol{X}}{\partial\boldsymbol{x}} = \frac{\partial \left( \boldsymbol{x} + \boldsymbol{u} \right)}{\partial\boldsymbol{x}} = \bold{I} + \nabla_{\boldsymbol{x}} \boldsymbol{u} ,
\end{equation}
where $\bold{I}$ is the second order identity and $\mathcal{W}$ is the stored-energy function, 
\begin{equation}
\mathcal{W} = \mathcal{W}_{dev} \left(\mathcal{F} \right) + \mathcal{W}_{vol} \left(J \right),
\label{eq:storedenergy}
\end{equation}
expressed in terms of a deviatoric term which depends on the deformation gradient
\begin{equation}
\mathcal{W}_{dev} \left(\mathcal{F} \right) = \frac{\mu}{2} \left( \text{tr} \left( \mathcal{\mathcal{F}^{T} \mathcal{F}} \right) -3 \right),
\end{equation}
and a volumetric term that depends on the volumetric deformation $J = \det \mathcal{F}$
\begin{equation}
\mathcal{W}_{vol} \left(J \right) = {\lambda}   \frac{\left(J^2 -1 \right)}{4} -  \left( \frac{\lambda}{2} + \mu \right) \ln \left( J \right)  .
\end{equation}
%
The stored-energy function $\mathcal{W}$ depends on two material parameters $\lambda , \mu > 0$ which are the Lamme constants \cite{SimoandHughes1998}, while the volumetric component depends on the logarithm of the volumetric strain $J$ to prevent the element flipping.  Combining Eqs. \eqref{eq:storedenergy} and \eqref{eq:PiolaKir}, the first Piola-Kirchhoff stress tensor is obtained
\begin{equation}
\displaystyle  \mathcal{P} \left( \boldsymbol{u} \right) = \lambda \frac{J^2 - 1}{2} \mathcal{F}^{-T} + \mu \left( \mathcal{F} - \mathcal{F}^{-T} \right).
\end{equation}
%
Considering that the proposed method solves an equation system explicitly, we decided to preserve the non-symmetric stress tensor in our calculations, since it just affect the right hand side and the formulation remains in terms of a mapping given by the deformation gradient. 
%
Once the  physical problem is presented, we adjust all these set of equations to fit them in the predictor multi-corrector time-integrator we presented previously. For solving the problem \eqref{eq:elastodynamic}, we can rewrite the bi-linear form \eqref{eq:ParabolicPDEproblem} as:
\begin{equation}
a \left( \boldsymbol{v}  ,  \boldsymbol{u}  \right) = \displaystyle  \left( \nabla_{\boldsymbol{x}} \boldsymbol{v} , \mathcal{P} \left( \boldsymbol{u} \right)  \right)_{\mathcal{B}_{0}} , 
\label{eq:FuncAHyper}
\end{equation}
while the linear term is 
\begin{equation}
\displaystyle  \left\langle  \boldsymbol{v} , \boldsymbol{f} \right\rangle =  \left\langle \boldsymbol{v}  , \rho_{0} \boldsymbol{g}  \right\rangle_{\mathcal{B}_{0}}  + \left(   \boldsymbol{v}  , \boldsymbol{t} \right)_{\partial \mathcal{B}_{0}} . 
\label{eq:RHShyper}
\end{equation}
%
It is worth to note that the first term in Eq. \eqref{eq:ParabolicPDEproblem}, related with the inertia effects, is multiplied by the density as $\left\langle \boldsymbol{v} , \rho_{0} \ddot{\boldsymbol{u}}  \right\rangle$ in order to obtain a proper mass matrix. To compute a proper bilinear functional, we deploy Gateaux derivative \cite{HUGHES1978391,BatheRamm1975} on Eq. \eqref{eq:FuncAHyper} and obtain:
\begin{equation}
\overrightarrow{a} \left( \boldsymbol{v}, \lJump \boldsymbol{u} \rJump ;  \boldsymbol{u}_{n} \right)  = \displaystyle \frac{d}{d\epsilon} a \left( \boldsymbol{v} , \boldsymbol{u}_{n} + \epsilon  \lJump \boldsymbol{u} \rJump  \right) \vert_{\epsilon=0} =  \left(  \nabla_{\boldsymbol{x}} \boldsymbol{v},   \left[ \frac{\partial \mathcal{P} \left( \boldsymbol{u} \right)}{\partial \mathcal{F}} \right]_{n} \nabla_{\boldsymbol{x}} \lJump \boldsymbol{u} \rJump   \right)_{\mathcal{B}_{0}} ,
\label{eq:FuncAHypergateaux}
\end{equation}
where the tangent constitutive hyperelastic tensor is computed through the following expression
\begin{equation}
\displaystyle \frac{\partial \mathcal{P} \left( \boldsymbol{u} \right)}{\partial \mathcal{F}} =  \mathcal{F}^{-1} \left[ \lambda J^{2} \bold{I} \otimes \bold{I} + 2 \mu \left( 1 + \frac{\lambda}{2 \mu} \left( 1 - J^2 \right)\right) \boldsymbol{1}  + \left( \mathcal{P} \left( \boldsymbol{u} \right) \mathcal{F}^{T} \right) \otimes \bold{I}\right]\mathcal{F}^{-T},
\end{equation}
where $\boldsymbol{1} = \frac{1}{2} \left( \delta_{ac} \delta_{bd} + \delta_{ad} \delta_{bc}\right)$ denots a symmetric fourth-order unit tensor with $ \delta_{ij}$ being a delta Kronecker function.
%
Finally, using Eqs. \eqref{eq:FuncAHyper}, \eqref{eq:RHShyper} and \eqref{eq:FuncAHypergateaux}, the update formulas presented in \eqref{eq:Galphau7} and \eqref{eq:Galphadotu1} can be used for the time-marching calculation.

